RLupus: Cooperation through emergent communication in The Werewolf social deduction game

This paper focuses on the emergence of communication to support cooperation in environments modeled as social deduction games (SDG), that are games where players communicate freely to deduce each others' hidden intentions. We first state the problem by giving a general formalization of SDG and a possible solution framework based on reinforcement learning. Next, we focus on a specific SDG, known as The Werewolf, and study if and how various forms of communication influence the outcome of the game. Experimental results show that introducing a communication signal greatly increases the winning chances of a class of players. We also study the effect of the signal's length and range on the overall performance showing a non-linear relationship.

==> reviews_answer1.tex <==
\section*{Reviews}

Dear Editors and Reviewers,\\
thank you very much for your detailed and very appropriate comments.
We took all of them in careful consideration and fully revised the paper to improve its quality.

Please find below the detailed answers to  all the comments received and explanations on how they have been considered in the revised version of this manuscript.

\paragraph{Q1}
\textit{ Page 5, RLupus Environment: 'Dealing with RL implies the presence
of action and state space', that should be given in a formal
definition, before talking specifically about the game. The one
given is not sufficient as already stated. }.

\textbf{Answer}
Added section 5.2 which intercedes the concept of action/observation space in relation with Markov decision processes.


\paragraph{Q2}
\textit{ Page 2, third paragraph: 'Shortly after' I would like to see at least one reference instead of this expression.}

\textbf{Answer}
Added citation to \cite{tampuu2017multiagent}

\paragraph{Q3}

\textit{Page 4: I have already spoken above about the section on the framework, but, just for instance, each party has to choose an
optimal policy while in the experiments is every agent choosing a policy. This section should be rewritten specifying better what a
policy is and contextualizing it in a RL framework.}

\textbf{Answer}
Thank you for spotting this.
We added definitions for two types of goals
\begin{itemize}
    \item Agent based \emph{micro-goal}:  is the main factor stirring the agent's behavior and it can be considered together with the other agents for cooperative games or alone for competitive ones.
    \item Party based \emph{macro-goal}: members of the same party have aligned interests that combined make up the party goal. 
\end{itemize}


\paragraph{Q4}
\textit{Page 4, second paragraph: The difference between implicit and explicit communication is used but not described.
}

\textbf{Answer}
We have clarified in the paper: "explicit communication as the act of sharing information for the sole purpose of affecting other agents’ mental state. On the other hand,  implicit  communication  regards  all  those types of actions that carry more than one meaning, e.g. guiding someone to a goal."



\paragraph{Q5}
\textit{I would avoid a phrase like 'relatively straightforward 'when the explanation is given mentioning a lot of concepts without giving a description.}

\textbf{Answer}
We removed the incorrect phrasing and further described the mentioned concepts.



\paragraph{Q6}
\textit{Page 3, in the problem Statement: is n the same for all $P^{(m)}$?}

\textbf{Answer}
No, it varies between parties, footnote included.


\paragraph{Q7}
\textit{Table 1 is referenced in the text after Table 2}

\textbf{Answer}
Table references have been fixed.

\paragraph{Q8}
\textit{how the state is observed by the players}

\textbf{Answer}
In the appendix \ref{app:obs_space}, we defined the complete observation state as well as the action one. The former is passed to each agent by the environment.


\paragraph{Q9}
\textit{For example why did the authors choose to use PPO instead of other algorithms or why didn't they compare it with other algorithms? PPO is presented in the Related Work section but not properly described.}

\textbf{Answer}
This is a good point indeed.
PPO was chosen for its widespread success in MAS environment \cite{wei2019mixed,guan2020centralized}, as included in this version. Comparison with other algorithms is left as future work. 


\paragraph{Q10}
\textit{Is there some specific reason to employ an LSTM rather than a fully connected network? Is this related to some form of partial observability?}

\textbf{Answer}
Indeed it is tied to the partial observability of the environment. We made this clear in Section \ref{sec:method:policy}

\paragraph{Q11}
\textit{the authors say in Sec 1 that "the reinforcement learning paradigm was not strong enough to be applied to a complex social  system. For this reason, researches [Schmidhuber, 2015] integrated RL with deep neural networks (DeepRL, DRL)." I think this sentence is misleading. The need for deep architectures derives from the complexity of the problem (the environment)rather than the fact that the algorithm will be applied to a social system.}

\textbf{Answer}
Indeed it was misleading, we rephrased it as: "the reinforcement learning paradigm may not scale up easily in complex multi-agent systems".

\paragraph{Q12}
\textit{ no explicit notion of "utility" for the players/parties}

\textbf{Answer}
We gave a better formulation which follows:
"the game evolves as a sequence of actions performed by the players of the parties, typically in turns.  The  effect  of  these  actions  contributes  to the definition of the game score. The  goal  of  each  party  is  to  maximize  some score, by performing suitable social behaviors, including,  for  example,  leveraging  other  players  by means of bluffs and lies."

\paragraph{Q13}
\textit{"S implementing the game logic?"}

\textbf{Answer}
Redefined with:
"The game evolves as a sequence of actions performed by the players of the parties, typically in turns.  The  effect  of  these  actions  contributes  to the definition of the game score"

\paragraph{Q14}
\textit{the authors say that they keep the policy of one party fixed while the one of the other is actually learning. I found this choice somehow limited, as the adversary nature of the interaction between the two parties is no longer present. I understand that the focus of the work is on communication, but I think that this should be made clear to understand the actual scope of application of MARL} 

\textbf{Answer}
We included a whole new paragraph at the end of Section \ref{sec:method:policy} in order to answer to this question, with the following content:
"Finally, we must address the possibility of an environment where both villagers and werewolves are able to learn. 
Having multiple agents learning at the same time void the stationary assumption which is necessary for optimality in RL. This assumption is already invalidated by the presence of multiple villagers but the coordination between them alleviates the problem. Introducing an adversarial set of learning agents would cause an increased complexity that would cloud the goal of this paper which is to study the emergence of a language between agents."

\paragraph{Q15}
\textit{How the actions (game and communication ones) influence these parts of the state, i.e. the transition model (which is just mentioned in Sec 4)}

\textbf{Answer}
We introduced a new paragraph in Section \ref{sec:method:env} to describe the transition model as follows: "The transition model fully depend on the target action, that is the environment is independent of the communication between agents. Indeed $S$ switches between night and day at every timestep $t$ and removes dead players from the environment."

\paragraph{Q16}
\textit{the policy takes as input a pair (game action, communication action) and provides as output a pair of the same kind. In RL, a policy takes as input a state and provides as output an action. How does this definition comply with the one presented in the paper? }

\textbf{Answer}
We defined the game/communication action pair in detail in the appendix \ref{app:obs_space}. 


\paragraph{Q17}
\textit{Page 3: All the speech is really too much informal. Phrases like 'some score', 'suitable behaviours' should be formalised in this section.}

\textbf{Answer}
Informal words have been replaced.


\paragraph{Q18}
\textit{it is not clear to me if, in such a way, we are forcing each agent to play a game action and a communication action simultaneously.}

\textbf{Answer}
We provided a better description in Section \ref{sec:method:env}:
"In a way, the agent can be seen as playing an action and communication game simultaneously. While this is the case for a \textit{communication turn} environment \ref{sec:framework:turns}, in a framework were signals are embedded in the action space the agent is free to take advantage of them or not based on its exploration phase."


\paragraph{Q19}
\textit{Page 3: The sections on MARL and Emergent Communication can be improved a lot in my opinion. I do not see any reference to many works about learning cooperation and communication in multi-agent deep RL, which are related to the topic of the work. I suggest the authors to look for example at this survey 10.1007/s10458-019-09421-1 (DOI).}

\textbf{Answer}
We rewrote the Related work altogether, now the emergent communication part has more suitable citations such as \cite{wagner2003progress,li2020emergent,lazaridou2020emergent,liang2020emergent,foerster2016learning,kottur2017natural,mordatch2018emergence}

\paragraph{Q20}
\textit{I would have appreciated a greater effort in order to explain the differences in outcome of the various models. Some hints are given but there is not a real discussion of that. Also the last section contains a comparison with the work of Kajibara et al. and it is not really clear to me if this is meaningful, since the authors themselves state that the results are not directly comparable.}

\textbf{Answer}
We rephrased the all section in order to make clear the similarity between the two methodologies as well as the different implementations that make the results not directly comparable.

\paragraph{Q21}
 \textit{Page 4: The definition of S, A and $C_ij$ is not sufficient in my opinion. formulation is unclear and does not provide all the formal elements}
 
\textbf{Answer}
We added a formalization for S,A,O and direct references to appendix where each space is defined.

\paragraph{Q22}
\textit{I think that the concept of SL and SR should be explained better maybe also in a technical way (for instance some implementation details).}


\textbf{Answer}
The concept of SR/SL have been explained in better details both with the introduction of Figure \ref{fig:signal}  and a description as follows:

"Indeed the action space is divided into two parts: 
\begin{itemize}
    \item \emph{Target}: The target $a_t$ is an integer in range $a_t \in [0,N-1]$, where $N$ is the number of players. Its intended usage is to allow players to vote for other players during the game. The range of possible values never changes during the execution, instead, illegal actions, such as voting for dead players, are filtered out later in the model. 
    \item \emph{Signal}: The signal vector $C^{(t)}$ \ref{fig:signal} is defined by two integer values: its length $SL \in [0,\infty[ $ which can be any value from zero (no communication) to an arbitrary large integer; its range $SR \in [2,N]$ that defines the number of possible values it can have. $SR$ is lower bounded to be 2, since a signal with only one possible value would be considered a static vector carrying no information; the upper bound $N$ comes from the necessity for the signal to be embedded with the target. Both are used in order to define the valid space for communication before training.
\end{itemize}
"


%\paragraph{Q}
%\textbf{Answer}



==> reviews_answer2.tex <==
\section*{Reviews}

Dear Editors and Reviewers,\\
we would like to thank you for the detailed and helpful comments.
We took all of them in careful consideration and fully revised the paper to improve its quality.

Please find below the detailed answers to  all the comments received and explanations on how they have been considered in the revised version of this manuscript.

\paragraph{Q1}
\textit{The formalization of Section 3 is clear, but why not using the same symbol $\mathcal{O}$ for the observation space also in Section 5.2 when introducing the MDP, instead of $\mathcal{M}$? Aren't they the same? }.

\textbf{Answer}
Indeed they are the same object, we replaced $\mathcal{M}$ with $\mathcal{O}$.


\paragraph{Q2}
\textit{I got confused in the paragraph "Observation Space" in Section 5.2, when it is said, "This space includes both the actions space and other information about the environment". Why does the observation space include the action space?}

\textbf{Answer}
By "This space includes both the actions space ..." we mean that the observation space includes information about other agents' actions.
We rephrased it to be more specific.

\paragraph{Q3}
\textit{The symbol P for the transition model makes confusion with the P of the "opposing parties"}

\textbf{Answer}
Changed to $\mathcal{T}$


\paragraph{Q4}
\textit{In relation to Q6, the authors specified that the number of players per party can vary. Still the notation is a simple "n" which is the same for every party. I understand the will of not complicating much the notation, but "n" should really be replaced by a "n(k)" or a similar expression, since it depends on "k".}

\textbf{Answer}
We added the following clarification in section \ref{sec:problem_stat} to avoid any kind of confusion:
\textit{"For the sake of conciseness, we drop the $k$ dependency and denote the number of players in a party as simply $n$"}


\paragraph{Q5}
\textit{In Section 5.2/5.3 there are some typos: "The action is processed by S which transition the the next state $m_{t+1}$ and yield a reward $r_t$ to the agent. This feedback loop continues until the agent reaches a terminal state and restarts.". It should be something like "…is processed by S which transitions to the…and
yields…". And: "In a way, the agent can be seen as playing an action $g_t$ and communication $c_t$ game simultaneously.", this sentence does not seem correct.}

\textbf{Answer}
Fixed thanks.

\paragraph{Q6}
\textit{ In Section 5.4 the description contains a typo "metric" should be plural, I guess}

\textbf{Answer}
We could not find the referenced word. 

\paragraph{Q7}
\textit{. Also in Learning Werewolves the sentence: "Finally, we must address the possibility of an environment where both villagers and werewolves are able to learn", seems really an answer to an unexpressed question (made in this case by reviewers). Please rephrase it.}

\textbf{Answer}
We introduced the question in a more explicit manner:
"Up until now, only villager agents have been able to learn from experience, while the werewolf behave according to a static policy."


\paragraph{Q8}
\textit{On a final note, the experiments are indeed explained better than in the first version, and there is one particular I am curious about, and I think is worth observing. In the 9 players case, the communication seems to affect the Suicide rates and the Villagers
Win Rate, more than the Accord (which seems almost unaffected by the insertion of communication, as one can see from Table 2).
This is more or less discussed in the Conclusions, where the authors argue how much the Suicide rate affects coordination "while keeping the accord to a maximum". I find this fact rather counterintuitive, and maybe a few more lines of discussion could be interesting for readers.}

\textbf{Answer}
%I don't really understand what is counterintuitive about it.
We would argue this observation is actually intuitive.
The communication allows the agent to explore the environment better thus making voting for oneself (suicide) a dominated action.



\paragraph{Q9}
\textit{In order to respond to Q3, the authors have distinguished between players' micro-goals and parties' macro-goals, which sounds fine. Anyway in Section 4 again, it is unclear who is optimizing which policy. I guess the policy defined in "Action Policy" is a single player's one, thus talking about optimal strategies for parties(like at the beginning of the section) seems confusing. I would like this section to be clear and not leave any kind of doubt to the reader, since it is an important part of the paper, as the authors say.
}

\textbf{Answer}
We introduced the following sentence in section 4 to be more specific about which goal is the policy pursuing:\\
\textit{Although the coordinated behavior favors the parties' macro-goal, the actual policy works on the players' micro-goal level.}
%\paragraph{Q}
%\textit{}
%\textbf{Answer}

==> todo.tex <==
\section*{TODO}

However, I still believe that the formalization of the problem, especially the connection between the notation used in Section 3 and Section 5.2, could be harmonized. Specifically:


\begin{enumerate}


\item In order to respond to Q3, the authors have distinguished between players' micro-goals and parties' macro-goals, which sounds fine.Anyway in Section 4 again, it is unclear who is optimizing which policy. I guess the policy defined in "Action Policy" is a single player's one, thus talking about optimal strategies for parties(like at the beginning of the section) seems confusing. I would like this section to be clear and not leave any kind of doubt to the reader, since it is an important part of the paper, as the authors say.



\end{enumerate}

